To Transmit or Not to Transmit: Optimal Sensor Schedule for Remote State Estimation of Discrete-Event Systems

This paper considers the problem of optimal sensor schedules for remote state estimation of discrete-event systems. In this setting, the sensors observe information from the plant and transmit the observable information to the receiver or estimator selectively. A transmission mechanism decides whether the observable information is transmitted or not, according to an information transmission policy, such that the receiver has sufficient information to satisfy the purpose of decision-making. To construct such a transmission mechanism, we first construct a non-deterministic dynamic observer that contains all feasible information transmission policies. Then, we show that the information updating rule of the dynamic observer indeed yields the state estimate from the receiver's point of view. Finally, we propose an approach to extract a specific information transmission policy, realized by a finite-state automaton, from the dynamic observer while satisfying some desired observation properties. To reduce transmission-related costs, we also require that the sensors transmit events as few as possible. A running example is provided to illustrate the proposed procedures.

==> sec2_probm.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminaries and Problem Formulation} \label{sec2_probm}

\subsection{System Model}
We consider a DES modeled by a deterministic finite-state automaton (DFA)
\begin{align*}
\textbf{G}=(Q,\Sigma,\delta,q_0),
\end{align*}
 where  
 $Q$ is a finite set of states, 
 $\Sigma$ is a finite set of events, 
 $\delta\colon Q\times \Sigma\to Q$ is a (partial) transition function,  
 $q_0\in Q$ is the initial state. 
 In the usual way, $\delta$ can be extended to $\delta\colon Q\times \Sigma^{*}\to Q$, where $\Sigma^{*}$ is the set of all finite-length {\it strings}, including the empty string $\varepsilon$. The {\it generated behavior} of $\bf{G}$ is language $L(\textbf{G})=\{s\in \Sigma^{*}: \delta(q_0,s)!\}$, where $\delta(q_0,s)!$ means that $\delta(q_0,s)$ is defined.

A string $s_1\in \Sigma^{*}$ is a {\it prefix\/} of $\textit{s}\in \Sigma^{*}$, written as $s_1\leq s$, if there is a string $s_2\in \Sigma^{*}$ such that $s_1s_2 = s$. The length of a string $s$ is denoted by $|s|$. The {\it prefix closure\/} of a language $L$ is the set $\overline{L} = \{s\in\Sigma^{*} :\exists t\in L \text{ s.t. } s\leq t\}$. For a natural number $n$, let $[1,n]=\{1,\ldots,n\}$ denote the set of all natural numbers from 1 to $n$. Let $\Sigma \subseteq\Sigma_{o}$, we denote by $P:\Sigma^*\to \Sigma_{o}^*$ the standard natural projection from $\Sigma$ to $\Sigma_{o}$.

The sensors transmit events dynamically based on the observation history. When the sensor corresponding to an event is transmitted after the occurrence of string $s$, the occurrence of this event is observable after $s$. Note that the observability of an event at different states may be different. 
Under dynamic sensing transmission decisions, the observations of the system behavior are specified by an \emph{information transmission policy}
\[
\omega: L(\bf{G})\rightarrow \Theta,
\]
where for any string $s\in L(\bf{G})$, $\omega(s)$ is the set of events that are transmitted after the occurrence of $s$. A projection based on a given information transmission policy $\omega$ is recursively defined by $P_{\omega}: L(\bf{G})\rightarrow \Sigma^*$
\[
P_{\omega}(\epsilon)=\epsilon; \\
  P_{\omega}(s\sigma)  =
  \begin{cases}
  P_{\omega}(s)\sigma, \mbox{if}\ \sigma\in \omega(s)\\
   P_{\omega}(s), \mbox{if}\ \sigma\notin \omega(s)
   \end{cases}
\]
We denote the set of all sensor transmission policies by $\Omega$. For any two sensor transmission policies $\omega_1, \omega_2\in \Omega$, we say $\omega_1$ is smaller than $\omega_2$, denoted by $\omega_1\less\ \omega_2$, if (1) $\forall s\in L(\bf{G}):\ \omega_1(s)\subseteq \omega_2(s)$; and (2) $\exists s\in L(\bf{G}):\ \omega_1(s)\subset \omega_2(s)$.

For any string $s\in L({\bf G})$  generated by the system, we define
\begin{align}
\mathcal{E}_{\Omega}^G(s):=\{\delta(q_0,t)\in Q : \exists t\in L({\bf G})\text{ s.t. }P_{\Omega}(s)=P_{\bar{\Omega}}(t)\} 
\end{align} 
as the central {\it state  estimate} of the system. 
Clearly, for  strings $s,t\in L({\bf G})$, if $P_{\Omega}(s)=P_{\Omega}(t)$, then   $\mathcal{E}_{\Omega}^G(s)=\mathcal{E}_{\Omega}^G(t)$.

 In this work, instead of considering specific objectives, e.g., control or diagnosis, we consider a general class of decision making requirement called the \emph{distinguishability}. 


\begin{Definition}(Distinguishability)
Let  $T\subseteq  Q\times Q$ be the specification imposed on the system  ${\bf G}=(Q,\Sigma, \delta, q_0)$, 
and $\bar{\Omega}=[\Omega_1,\Omega_2,\dots ,\Omega_n]$ be a set of information transition policies. 
We say that ${\bf G}$ is distinguishable w.r.t. $\bar{\Omega}$ and $T$ if for any string $s\in L({\bf G})$, we have
  \begin{align}
   (\mathcal{E}_{\bar{\Omega}}^G(s)\times \mathcal{E}_{\bar{\Omega}}^G(s)) \cap T =\emptyset.
 \end{align} 
\end{Definition} 
\medskip 

In the above definition, specification $T$ is a set of state pairs for which the central site should always be able to distinguish, i.e.,  for any $(x, x')\in T$, if $x$ is possible in the state estimate, then $x'$ should not be included in it, and vice versa. 

Our objective is to synthesize a information transmission policy such that some given property holds. We define the Minimal Information Transmission Problem as follows.
\begin{Porblem}\label{problem1}
 Given a plant $\textbf{G}=(Q,\Sigma,\delta,q_0)$  and $T\subseteq Q\times Q$ be a specification.  Find a information transmission policy $\omega\in \Omega$ s.t. (i) ${\bf G}$ is distinguishable w.r.t. $\omega$ and $T$.; (ii) $\nexists \omega'\in \Omega$ s.t. $\omega'\less\ \omega$.
 \end{Porblem}

\subsection{A general most comprehensive dynamic observer}
For implementation purposes, we need to build a finite representation of the function $\Omega$. To this end, we define the structure of dynamic observer that realizes all sensor activation policies.


We recall the definition of  nondeterministic finite-state automaton (NFA)
\begin{align*}
\textbf{G}=(Q,\Sigma,\delta,q_0),
\end{align*}
 where  
 $Q$ is a finite set of states, 
 $\Sigma$ is a finite set of events, 
 $\delta\colon Q\times \Sigma\to Q$ is a (partial) transition function,  
 $q_0\in Q$ is the initial state. 


% That is, for the observation $s\sigma \in \Sigma_{o}^*\Sigma_{o}$, $\Omega$ will decide whether to transmit the observation of $\sigma$, i.e., $\Omega(s\sigma)=\sigma$, or not, i.e., $\Omega(s\sigma)=\epsilon$. The above definition of information transmission policy is history dependent. 

We attach the information transmission policy to the system \textbf{G}, which can be represented as a nondeterministic finite-state automaton (NFA)
\begin{align}
{\bf G}_{ag}=(\tilde{Q},\Sigma_o,f,\tilde{q_{0}}),
\end{align}
where 
\begin{itemize}
    \item 
    $\tilde{Q}=2^Q\times L^{|\Sigma_o|}$ is the state set and $L: X \times \Sigma_{o}\rightarrow  \{Y, N\}$ is a labeling function that determines whether the current observable event is transmitted (Y) or not (N);
    \item 
    $\Sigma_o\subseteq \Sigma$ is the event set;
    \item 
    $f:\tilde{Q}\times \Sigma_o\to \tilde{Q}$ is the partial transition function defined by: for any $\tilde{\imath},\tilde{\imath'}\in \tilde{Q}$, $\sigma \in \Sigma_o$, we have $f(\tilde{\imath},\sigma)=\tilde{\imath'}$ iff
    \begin{align}
   \tilde{\imath'}=UR(NX_{\sigma}(\tilde{\imath}))
    \end{align}
where for any $\tilde{\imath}\in 2^{Q}$, $\sigma \in \Sigma_o$, we have 
\[
   NX_{\sigma}(\tilde{\imath})=\{q'l_{q'}\in \tilde{Q}:\ \exists\ ql_{q}\in \tilde{\imath}\ s.t.\ \delta(q,\sigma)=q' \}
 \]
 \[
   UR(\tilde{\imath})=\{q'l_{q'}\in \tilde{Q}:\ \exists\ ql_{q}\in \tilde{\imath},\ \exists\ s\in (\Sigma\setminus \Sigma_o)^*\ s.t.\ \delta(q,s)=q' \}
\]
    with $l_{q}=\{Y,N\}^{|E_{q}|}$ and $E_{q}=\{\sigma\in \Sigma|\delta(q,\sigma)!\}$ is the set of events that are defined at state $q$ in \textbf{G}.
    \item 
    $\tilde{q_{0}}=UR(NX_{\sigma}(\tilde{q_0}))$ is the initial state, where $\tilde{q_0}=q_0\times \{Y,N\}^{|E_{q_0}|}$. 
\end{itemize}
 \begin{figure}
  \centering
  \includegraphics[width=0.4\textwidth]{G.pdf}\\
  \caption{The plant and the observer for \textbf{G}}
  \label{fig:G}
\end{figure}
An illustrative example is given in Fig.~\ref{fig:G}.

To solve Problem~\ref{problem1}, we construct a dynamic observer of ${\bf G}_{ag}$, which  needs the following definitions.

\begin{Definition}{}
Let $\imath=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in 2^{\tilde{Q}}$. We say $\imath$ is 
{\it unobservable reachable} if 

$\forall q_il_{q_i}\in \imath$: $\exists\ q_{j1}l_{q_{j1}},q_{j2}l_{q_{j2}},\dots,q_{jm}l_{q_{jm}} \in \imath$, $\sigma_i\in \Sigma_o$ with $l_{q_{j1}}=l_{q_{j2}}=\dots=l_{q_{jm}}=N$ and $\delta(q_{ji},\sigma_i)=q_{ji+1}$ s.t. $\delta (q_{j1},\sigma_1\sigma_2,\dots,\sigma_m)=q_i$.
\end{Definition}

\begin{Definition}{}
Let $\imath=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in 2^{\tilde{Q}}$. We say $\imath$ is 
{\it unobservable reach-closed} if 

$\forall q_il_{q_i}\in \imath$ with $l_{q_i}=N$: $\exists\ q_jl_{q_j} \in\ \imath$ s.t. $\delta (q_i,\sigma)=q_j$.
\end{Definition}

\begin{Definition}{}
Let $\imath=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in 2^{\tilde{Q}}$. We say $\imath$ is 
{\it decision consistent} if 

$\forall q_il_{q_i}\neq q_jl_{q_j}\in \imath$: $\exists\ s^{\imath}_1,s^{\imath}_2\in \Sigma_o^*$ and $q_{\ell}l_{q_{\ell}}\in \imath$ s.t. $\delta (q_{\ell}l_{q_{\ell}},s^{\imath}_1)=q_il_{q_i}$, $\delta (q_{\ell}l_{q_{\ell}},s^{\imath}_2)=q_jl_{q_j}$, and $s^{\imath}_1\neq s^{\imath}_2$.
\end{Definition}



Now we construct the dynamic observer of ${\bf G}_{ag}$, which is defined as a new NFA
\begin{align}\label{observer g}
Obs({\bf G}_{ag})=(Z,\Sigma_o,\xi,z_{0}),
\end{align}
where 
\begin{itemize}
    \item 
$Z\subseteq 2^{\tilde{Q}}$ is the set of states, 

\item
$\Sigma_o$ is the set of events, 

\item
$\xi: Z\times \Sigma_o \to Z$ is the partial transition function defined by: 
for any $z\in Z, \sigma\in \Sigma$, we have 
\[
\xi(z,\sigma)= U\!R( N\!X_{\sigma} (z )),
\]
where for any $z\in Z$, we have $z'=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in N\!X_{\sigma} (z )$ iff
\begin{align}
    \{q_1,q_2,\dots, q_k\}=\{q\in Q: \exists q'l_{q'}\in z\ s.t.\ L(q',\sigma)=Y \& \delta(q',\sigma)=q\}
\end{align}
and $z'=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in U\!R(z)$ iff $z'$ is {\it unobservable reachable}, {\it unobservable reach-closed}, and decision consistent.

\item
$z_0=UR(NX_{\sigma}(\tilde{q_0}))$ is the initial state. 
 \end{itemize}
 
The initial state $z_0$ is defined by $U\!R( \{\tilde{q_0}\} )$. 
Intuitively,  $ N\!X_{\sigma} (z)$ is the set of states that can be reached from some state in $z$ immediately by transmitted event $\sigma$ and $U\!R(z)$ is the set of states that can be reached unobservably from some state in $z$. 

By condition (i) in Problem~\ref{problem1}, we must find a information transmission policy $\omega$ such that ${\bf G}$ is distinguishable w.r.t. $\omega$ and $T$. To this end, we need to delete all states that make the system ${\bf G}$ is undistinguishable and obtain a smaller dynamic observer $sub(Obs({\bf G}_{ag}))=(Z',\Sigma_o,\xi,z'_{0})$, where 
\[
Z'=Z\setminus \{\imath=\{q_1l_{q_1},q_2l_{q_2},\dots, q_kl_{q_k}\}\in Z:  \{q_1,q_2,\dots, q_k\}\cap T\neq \emptyset\}.
\]

In order to find a minimal information transmission policy as formulated in Problem 1 (condition (ii)), Algorithm 1 is provided to synthesize an deterministic supervisor which represents this minimal policy.

